Qualit\"atsma{\ss}e bin\"arer Klassifikationen im Bereich kriminalprognostischer Instrumente der vierten Generation

This master's thesis discusses an important issue regarding how algorithmic decision making (ADM) is used in crime forecasting. In America forecasting tools are widely used by judiciary systems for making decisions about risk offenders based on criminal justice for risk offenders. By making use of such tools, the judiciary relies on ADM in order to make error free judgement on offenders. For this purpose, one of the quality measures for machine learning techniques which is widly used, the $AUC$ (area under curve), is compared to and contrasted for results with the $PPV_k$ (positive predictive value). Keeping in view the criticality of judgement along with a high dependency on tools offering ADM, it is necessary to evaluate risk tools that aid in decision making based on algorithms. In this methodology, such an evaluation is conducted by implementing a common machine learning approach called binary classifier, as it determines the binary outcome of the underlying juristic question. This thesis showed that the $PPV_k$ (positive predictive value) technique models the decision of judges much better than the $AUC$. Therefore, this research has investigated whether there exists a classifier for which the $PPV_k$ deviates from $AUC$ by a large proportion. It could be shown that the deviation can rise up to 0.75. In order to test this deviation on an already in used Classifier, data from the fourth generation risk assement tool COMPAS was used. The result were were quite alarming as the two measures derivate from each other by 0.48. In this study, the risk assessment evaluation of the forecasting tools was successfully conducted, carefully reviewed and examined. Additionally, it is also discussed whether such systems used for the purpose of making decisions should be socially accepted or not.

==> template/de/rrlab_secondpage.tex <==
\thispagestyle{empty}

\begin{center}
  \vbox{
    \ificsecondpage{
      \advance\hsize by +2cm
    }
    \vspace{3cm}
    \vbox{\huge \RRLABVARtype}
    \vspace{3.5cm}
    \vbox{\parbox{12cm}{\centering \bf \LARGE \RRLABVARtitle}}
    \vspace{3.5cm}
    \vbox{\large %\RRLABVARinstitution 
		Algorithm Accountability Lab\\
     Fachbereich Informatik \\
       TECHNISCHE UNIVERSIT\"AT KAISERSLAUTERN
      }
	  \vspace{1cm}
    \vbox{\LARGE \RRLABVARauthor}
		\vbox{\url{krafft@cs.uni-kl.de}}
		\vbox{OrcID: 0000-0002-3527-1092 }
    \vspace{2cm}
    \vspace{\fill}
    \ifdipl{
      \vbox{
        \begin{tabular}[c]{lcl}
          {\bf Tag der Ausgabe} & : & \RRLABVARinception \\
          {\bf Tag der Abgabe}  & : & \RRLABVARsubmission \\ \\ \\
          {\bf Gutachter} & : & \RRLABVARfirstreviewer \\
          {\bf Betreuer} & : & \RRLABVARsupervisor \\
        \end{tabular}
      }
    }
    {
      \vbox{
        \begin{tabular}[c]{lcl}
          {\bf Tag der Ausgabe} & : & \RRLABVARinception \\
          {\bf Tag der Abgabe}  & : & 12. Mai 2017 \\ \\ \\
          {\bf Erstgutachter} & : & \RRLABVARfirstreviewer \\
          {\bf Zweitgutachter} & : & \RRLABVARsecondreviewer \\
        \end{tabular}
      }
    }
  }
\end{center}

\clearpage


==> template/de/rrlab_titlepage.tex <==
\thispagestyle{empty}
\newcommand{\HRule}{\rule{\linewidth}{1mm}}


  \begin{center}
    \vbox{
      \begin{center}
      \Large \bf %\RRLABVARinstitution
			\Large \bf \protect{ALGORITHM ACCOUNTABILITY LAB} \\
         \Large \bf \protect{FACHBEREICH INFORMATIK} \\
         \Large \bf \protect{TECHNISCHE UNIVERSIT\"AT KAISERSLAUTERN}
      \end{center}
    }
  \end{center}

\protect{ \HRule \vspace{0.5cm} }
\protect{ \vbox{\centerline{\Huge \bf \RRLABVARtype}}}

\protect{
  \vspace{0.15cm}
  \HRule
  \vspace{0.5mm}
}

\begin{center}
  \vbox{ \RRLABVARtitleimage }
  \vfill
  \vspace{0.8cm}
  \vbox{\bf \huge \RRLABVARtitle}
  \vspace{1cm}
  \vbox{\bf \huge \RRLABVARauthor}
  \vspace{0.6cm}
  
  \protect{ \HRule \vspace{0.3cm}}
  \protect{\vbox{ \bf \huge 12. Mai 2017}\vspace{0.1cm}}
  \protect{ \HRule }
\end{center}
\clearpage
 
\clearpage

